On Coding Efficiency for Flash Memories

Recently, flash memories have become a competitive solution for mass storage. The flash memories have rather different properties compared with the rotary hard drives. That is, the writing of flash memories is constrained, and flash memories can endure only limited numbers of erases. Therefore, the design goals for the flash memory systems are quite different from these for other memory systems. In this paper, we consider the problem of coding efficiency. We define the "coding-efficiency" as the amount of information that one flash memory cell can be used to record per cost. Because each flash memory cell can endure a roughly fixed number of erases, the cost of data recording can be well-defined. We define "payload" as the amount of information that one flash memory cell can represent at a particular moment. By using information-theoretic arguments, we prove a coding theorem for achievable coding rates. We prove an upper and lower bound for coding efficiency. We show in this paper that there exists a fundamental trade-off between "payload" and "coding efficiency". The results in this paper may provide useful insights on the design of future flash memory systems.

==> flash_memory_main_bib.tex <==



\begin{thebibliography}{99}

%\small

%\footnotesize


%\setlength{\parskip}{0pt}








\bibitem{Kuznetsov74} A. Kuznetsov and B. Tsybakov, ``Coding in a memory with defective
cells'', Problems of Information Transmission, 1974,  vol. 10, no.
2, pp. 132-138, 1974.



\bibitem{Heegard83} C. Heegard
``Partitioned linear block codes for computer memory with 'stuck-at'
defects'', IEEE Transactions on Information Theory, vol. 29, pp.
831-842, 1983.





\bibitem{Heegard83b} C. Heegard, and A. El-Gamal, ``On the capacity of computer memory
with defects'', IEEE Transactions on Information Theory, vol. 29,
pp. 731-739, 1983.



\end{thebibliography}

































%

